Knowledge Distillation for Quality Estimation

Quality Estimation (QE) is the task of automatically predicting Machine Translation quality in the absence of reference translations, making it applicable in real-time settings, such as translating online social media conversations. Recent success in QE stems from the use of multilingual pre-trained representations, where very large models lead to impressive results. However, the inference time, disk and memory requirements of such models do not allow for wide usage in the real world. Models trained on distilled pre-trained representations remain prohibitively large for many usage scenarios. We instead propose to directly transfer knowledge from a strong QE teacher model to a much smaller model with a different, shallower architecture. We show that this approach, in combination with data augmentation, leads to light-weight QE models that perform competitively with distilled pre-trained representations with 8x fewer parameters.

==> tables/data.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lr@{}}
\toprule
Language & Sentences \\
\midrule
Estonian & 25,176 \\
Romanian & 372,690 \\
Sinhala & 139,406 \\
Nepalese & 85,343 \\
English & 1,563,519 \\
\bottomrule
\end{tabular}
\caption{Number of sentences extracted from Wikipedia for data augmentation.}
\label{tab:data}
\end{table}


==> tables/distillBySize.tex <==
%\begin{table}[ht!]
%    \centering \small
%    \begin{tabular}{@{}lcccc@{}}
%    \toprule
%     & Ro-En & Si-En & Ne-En & En-Zh \\
%    \midrule
%Wiki-dist-10K-random & 0.5597 ±0.00428 & 0.3644 ±0.00314 & 0.4072 ±0.00168 & 0.09444 %±0.0108 \\
%
%%Wiki-dist-30K-random & 0.63 & 0.42 & 0.51 & 0.18 \\
%
%Wiki-dist-50K-random & 0.6447 ±0.00249 & 0.4492 ±0.0121 & 0.5256 ±0.0031 & 0.1968 %±0.0254 \\
%
%Wiki-dist-70K-random & 0.6581 ±0.00356 & 0.4627 ±0.0127 & 0.5363 ±0.00464 & 0.1891 %±0.0189 \\
%
%Wiki-dist-100K-random & 0.6867 ±0.00344 & 0.4696 ±0.0187 & 0.5433 ±0.00147 & 0.1674 %±0.015 \\
%\bottomrule
%\end{tabular}
%\caption{Pearson correlation on the test partition of the MLQE dataset for BiRNN %student models trained with different amounts of distilled data.}
%\label{tab:distillBySize}
%\end{table}

\begin{table}[t]
    \centering \small
    \begin{tabular}{@{}lcccc@{}}
    \toprule
     & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
10K & 0.56 ±.00 & 0.36 ±.00 & 0.41 ±.00 & 0.09 ±.01 \\
%Wiki-dist-30K-random & 0.63 & 0.42 & 0.51 & 0.18 \\
50K & 0.64 ±.00 & 0.45 ±.01 & 0.53 ±.00 & 0.20 ±.03 \\
70K & 0.66 ±.00 & 0.46 ±.01 & 0.54 ±.00 & 0.19 ±.02 \\
100K & 0.69 ±.00 & 0.47 ±.02 & 0.54 ±.00 & 0.17 ±.02 \\
\bottomrule
\end{tabular}
\caption{Pearson correlation on the test partition of the MLQE dataset for BiRNN student models trained with different amounts of distilled Wikipedia data.}
\label{tab:distillBySize}
\end{table}


==> tables/distillation.tex <==
\begin{table*}[t]
    \centering \small
    \begin{tabular}{@{}llccccc@{}}
    \toprule
    Name    & Training data & Et-En & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
    TQ$\mathrm{_{TEACHER}}$ & MLQE-gold & 0.77 & 0.88 & 0.60 & 0.75 & 0.44 \\
\cmidrule{1-7}
BiRNN$\mathrm{_{STUDENT}}$ & MLQE-dist & 0.40 & 0.51 & 0.41 & 0.41 & 0.18 \\
BiRNN$\mathrm{_{STUDENT+AUG100K}}$ & Wiki-dist & {\bf 0.49} & {\bf 0.72} & {\bf 0.48} & {\bf 0.57} & {\bf 0.26} \\
\cmidrule{1-7}
BiRNN$\mathrm{_{STUDENT+AUG10K}}$ & Wiki-dist & 0.41 & 0.41 & 0.27 & 0.33 & 0.06 \\
BiRNN$\mathrm{_{STUDENT+AUG10K+CONF}}$ & Wiki-dist & 0.41 & 0.54 & 0.36 & 0.37 & 0.15 \\
\cmidrule{1-7}
BiRNN & MLQE-gold & 0.30 & 0.51 & 0.35 & 0.35 & 0.20 \\
Predictor-Estimator & MLQE-gold & 0.48 & 0.69 & 0.37 & 0.39 & 0.19 \\
TQ$\mathrm{_{DistilBERT}}$ & MLQE-gold & 0.62 & 0.78 & 0.51 & 0.61 & 0.36 \\
    \bottomrule
    \end{tabular}
    \caption{Pearson correlation with human judgments on the test partition of MLQE. MLQE-gold refers to the training partition of MLQE dataset. MLQE-dist is the distilled version of the MLQE training set where teacher predictions are used as quality labels. Wiki-dist refers to the Wikipedia dataset produced by data augmentation. % Underlined results correspond to the teacher model, while
    Results marked in bold indicate our best distilled student models.}
    \label{tab:distillation}
\end{table*}


% \begin{table*}[t]
%    \centering \small
%    \begin{tabular}{@{}lllccccc@{}}
%    \toprule
%    Name    & Architecture  & Training data & Et-En & Ro-En & Si-En & Ne-En & En-Zh \\
%    \midrule
%    TQ$\mathrm{_{TEACHER}}$ & TQ (XLM-R) & MLQE-gold & 0.77  & 0.88  & 0.60 & 0.75 & 0.44\\
%\cmidrule{1-8}
%BiRNN$\mathrm{_{STUDENT}}$ & BiRNN & MLQE-dist & 0.40 & 0.51 & 0.41 & 0.41 & 0.18 \\
%BiRNN$\mathrm{_{STUDENT+AUG100K}}$ & BiRNN & Wiki-dist & 0.49 & 0.72 & 0.48 & 0.57 &  %\\
%\cmidrule{1-8}
%BiRNN$\mathrm{_{STUDENT+AUG10K}}$ & BiRNN & Wiki-dist-10K & - & 0.41 & 0.27 & 0.33 & 0.06 \\
%BiRNN$\mathrm{_{STUDENT+AUG10K+CONF}}$ & BiRNN & Wiki-dist-10K-conf & - & 0.54 & 0.36 & 0.37 & 0.15 \\
%\cmidrule{1-8}
%BiRNN & BiRNN & MLQE-gold & 0.30 & 0.51 & 0.35 & 0.35 & 0.20 \\
%OpenKiwi & OpenKiwi & MT training+MLQE-gold & 0.48 & 0.69 & 0.37 & 0.39 & 0.19 \\
%TQ$\mathrm{_{DistilBERT}}$ & TQ (DistilBERT) & MLQE-gold & 0.62 & 0.78 & 0.51 & 0.61 & 0.36 \\
%    \bottomrule
%    \end{tabular}
%    \caption{Distillation. TransQuest (TQ).\footnote{We exclude En-De from our experiments, as the performance of the available TQ models for this language pair is too low.}}
%    \label{tab:distillation}
%\end{table*}


==> tables/distillation_by_size.tex <==
\begin{table}[ht!]
    \centering \small
    \begin{tabular}{@{}lcccc@{}}
    \toprule
     & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
Wiki-dist-10K-random & 0.41 & 0.27 & 0.33 & 0.06 \\
Wiki-dist-30K-random & 0.63 & 0.43 & 0.41 & 0.18 \\
Wiki-dist-50K-random & 0.67 & 0.45 & 0.54 & 0.24 \\
Wiki-dist-70K-random & 0.68 & 0.46 & 0.56 & 0.27 \\
Wiki-dist-100K-random & 0.72 & 0.48 & 0.57 & 0.26 \\
\cmidrule{1-5}
Wiki-dist-10K-filtered & 0.54 & 0.36 & 0.37 & 0.15 \\
Wiki-dist-30K-filtered & 0.64 & 0.42 & 0.49 & 0.18 \\
Wiki-dist-50K-filtered & 0.69 & 0.45 & 0.52 & 0.19 \\
\bottomrule
\end{tabular}
\caption{Pearson correlation with human judgments on the test partition of the MLQE dataset for BiRNN student models trained with different amounts of distilled data, with and without noise filtering.}
\label{tab:filtering}
\end{table}


==> tables/efficiency.tex <==
\begin{table}[tb]
    \centering \small
    \begin{tabular}{@{}lrp{.8cm}p{1cm}p{.8cm}@{}}
    \toprule
            &           &  \multicolumn{2}{c}{Inference} \\
    \cmidrule(lr){3-4}
    Name    & \#params & Speed (secs.) & RAM (MiB) & Disk (M) \\
    \midrule
TQ$_{\mathrm{XLM-R-Large}}$  & 561M  & 0.82 & 9,263.5  & 2140 \\
TQ$_{\mathrm{DistilBERT}}$   & 135M  & 1.09 & 1,979.2  & ~~517 \\
BiRNN                        &  18M  & 0.39 & ~~155.6 & ~~132 \\
    
    \bottomrule
    \end{tabular}
    \caption{Efficiency. Inference speed and RAM for prediction are for 1 sentence on CPU (Intel Xeon Silver 4114 CPU @ 2.20GHz).}
    \label{tab:efficiency}
\end{table}


==> tables/newImpleDistillation.tex <==
\begin{table*}[t!]
    \centering \small
    \begin{tabular}{@{}llccccc@{}}
    \toprule
    Name    & Training data & Et-En & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
    TQ$\mathrm{_{TEACHER}}$ & MLQE-gold & 0.77 & 0.88 & 0.60 & 0.75 & 0.44 \\
\cmidrule{1-7}
BiRNN$\mathrm{_{STUDENT}}$ & MLQE-dist & 0.45 & 0.62 & 0.44 & 0.46 & {\bf 0.18} \\
BiRNN$\mathrm{_{STUDENT+AUG}}$ & Wiki-dist & {\bf 0.50} & {\bf 0.69} & {\bf 0.45} & {\bf 0.54} & { 0.17} \\
\cmidrule{1-7}
%BiRNN$\mathrm{_{STUDENT+AUG10K}}$ & Wiki-dist & 0.0.08 & 0.56 & 0.39 & 0.40 & 0.08 \\
%BiRNN$\mathrm{_{STUDENT+AUG10K+CONF}}$ & Wiki-dist & 0.41 & 0.54 & 0.36 & 0.37 & 0.15 \\
\cmidrule{1-7}
BiRNN & MLQE-gold & 0.37 & 0.60 & 0.40 & 0.42 & 0.15 \\
Predictor-Estimator & MLQE-gold & 0.48 & 0.69 & 0.37 & 0.39 & 0.19 \\
TQ$\mathrm{_{DistilBERT}}$ & MLQE-gold & 0.62 & 0.78 & 0.51 & 0.61 & 0.36 \\
    \bottomrule
    \end{tabular}
    \caption{Pearson correlation with human judgments on the MLQE test set. MLQE-gold:  training partition of MLQE dataset; MLQE-dist: distilled version of the MLQE training set with teacher predictions  used as labels;  Wiki-dist: the Wikipedia dataset produced by data augmentation. % Underlined results correspond to the teacher model, while
    Boldface results indicate our best student models.}
    \label{tab:distillation}
\end{table*}

==> tables/newImpleDistillation_by_size.tex <==
\begin{table}[ht!]
    \centering \small
    \begin{tabular}{@{}lcccc@{}}
    \toprule
     & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
Wiki-dist-10K-random & 0.56 & 0.39 & 0.40 & 0.08 \\
Wiki-dist-30K-random & 0.63 & 0.42 & 0.51 & 0.18 \\
Wiki-dist-50K-random & 0.64 & 0.45 & 0.52 & 0.16 \\
Wiki-dist-70K-random & 0.67 & 0.46 & 0.54 & 0.20 \\
Wiki-dist-100K-random & 0.69 & 0.45 & 0.54 & 0.17 \\
\cmidrule{1-5}
Wiki-dist-10K-filtered & 0.54 & 0.36 & 0.37 & 0.15 \\
Wiki-dist-30K-filtered & 0.64 & 0.42 & 0.49 & 0.18 \\
Wiki-dist-50K-filtered & 0.69 & 0.45 & 0.52 & 0.19 \\
\bottomrule
\end{tabular}
\caption{New Implementation Results}
\label{tab:newImpleFiltering}
\end{table}


==> tables/newValidDataSetDistillationBySize.tex <==
\begin{table}[ht!]
    \centering \small
    \begin{tabular}{@{}lcccc@{}}
    \toprule
     & Ro-En & Si-En & Ne-En & En-Zh \\
    \midrule
Wiki-dist-10K-random & 0.56 & 0.39 & 0.40 & 0.08 \\
Wiki-dist-30K-random & 0.63 & 0.42 & 0.51 & 0.18 \\
Wiki-dist-50K-random & 0.64 & 0.45 & 0.52 & {\bf 0.21} \\
Wiki-dist-70K-random & 0.67 & 0.46 & 0.54 & - \\
Wiki-dist-100K-random & 0.69 & 0.45 & 0.54 & - \\
\cmidrule{1-5}
Wiki-dist-10K-filtered & 0.54 & 0.36 & 0.37 & 0.15 \\
Wiki-dist-30K-filtered & 0.64 & 0.42 & 0.49 & 0.18 \\
Wiki-dist-50K-filtered & 0.69 & 0.45 & 0.52 & 0.19 \\
\bottomrule
\end{tabular}
\caption{New Implementation Different Valid Set Results}
\label{tab:newImpleFiltering}
\end{table}

